An efficient distributed learning algorithm based on effective local functional approximations

Scalable machine learning over big data is an important problem that is receiving a lot of attention in recent years. On popular distributed environments such as Hadoop running on a cluster of commodity machines, communication costs are substantial and algorithms need to be designed suitably considering those costs. In this paper we give a novel approach to the distributed training of linear classifiers (involving smooth losses and L2 regularization) that is designed to reduce the total communication costs. At each iteration, the nodes minimize locally formed approximate objective functions; then the resulting minimizers are combined to form a descent direction to move. Our approach gives a lot of freedom in the formation of the approximate objective function as well as in the choice of methods to solve them. The method is shown to have $O(log(1/\epsilon))$ time convergence. The method can be viewed as an iterative parameter mixing method. A special instantiation yields a parallel stochastic gradient descent method with strong convergence. When communication times between nodes are large, our method is much faster than the Terascale method (Agarwal et al., 2011), which is a state of the art distributed solver based on the statistical query model (Chuet al., 2006) that computes function and gradient values in a distributed fashion. We also evaluate against other recent distributed methods and demonstrate superior performance of our method.

==> relatedwork.tex <==
\section{Related work}

Quickly review IPM, terascale etc. already covered in section~\ref{intro}.

The ADMM method~\cite{Boyd2011}, like our method, solves approximate problems in the nodes and iteratively reaches the full batch solution. But it has the following disadvantages: (a) it does not have {\it glrc}; (b) the approximation problems are dictated by the ADMM formulation and so there is little flexibility; (c) the approximation problems need to be solved precisely; and (d) its efficiency is sensitive to the choice of the penalty parameter which is problem dependent.

Make sure to mention Deng \& Yin paper~\cite{deng2012} giving linear rate of convergence for ADMM.

Below are the comments on ADMM we wrote in the ICML rebuttal.

In our experience, ADMM is unsatisfactory; the penalty parameter ($\beta$ in Deng and Yin~\cite{deng2012}) creates difficulties. We actually did experiments on ADMM and observed the following.
\begin{itemize}
\item The recommended value of $\beta$ in Deng and Yin~\cite{deng2012} makes ADMM an order of magnitude slower than our method;
\item If $\beta$ is chosen to be the best possible value, ADMM works well;
\item The $\beta$ recommended by Deng and Yin~\cite{deng2012} is more than $10^4$ times this best value;
\item Even around this best value, the performance of ADMM is sensitive to the variation of $\beta$.
\item The optimal value of $\beta$ is also problem dependent. We are not aware of any efficient ways of automatically setting $\beta$ to good values. Nevertheless, we will include ADMM results when we revise the paper.
\end{itemize}

The ICML reviewers also asked about PDP book~\cite{bertsekas1997}. I have copied our response below.

Methods for separable convex programming given in Bertsekas and Tsitsiklis~\cite{bertsekas1997} are based on proximal and Augmented Lagrangian ideas. ADMM represents the best of these methods. Gauss-Seidel and Jacobi methods are related to feature partitioning, which is not the main theme of this paper. 

Mairal's MISO algorithm~\cite{mairal2013} is not meant for parallel solution. The main idea of MISO (which is in the spirit of the EM algorithm) is to build majorization approximations with good properties so that line search can be avoided, which is interesting. A distributed version of MISO is an interesting future direction, but, given that line search is inexpensive communication-wise, it is unclear if such a research direction would give great benefits.


